PixMatch: Unsupervised Domain Adaptation via Pixelwise Consistency Training

Unsupervised domain adaptation is a promising technique for semantic segmentation and other computer vision tasks for which large-scale data annotation is costly and time-consuming. In semantic segmentation, it is attractive to train models on annotated images from a simulated (source) domain and deploy them on real (target) domains. In this work, we present a novel framework for unsupervised domain adaptation based on the notion of target-domain consistency training. Intuitively, our work is based on the idea that in order to perform well on the target domain, a model's output should be consistent with respect to small perturbations of inputs in the target domain. Specifically, we introduce a new loss term to enforce pixelwise consistency between the model's predictions on a target image and a perturbed version of the same image. In comparison to popular adversarial adaptation methods, our approach is simpler, easier to implement, and more memory-efficient during training. Experiments and extensive ablation studies demonstrate that our simple approach achieves remarkably strong results on two challenging synthetic-to-real benchmarks, GTA5-to-Cityscapes and SYNTHIA-to-Cityscapes. Code is available at: https://github.com/lukemelas/pixmatch

==> intro.tex <==

\begin{abstract}

    % TODO: Change abstract
   Unsupervised domain adaptation is a promising technique for semantic segmentation and other computer vision tasks for which large-scale data annotation is costly and time-consuming. In semantic segmentation particularly, it is attractive to train models on annotated images from a simulated (source) domain and deploy them on real (target) domains. In this work, we approach unsupervised domain adaptation for semantic segmentation using recent ideas 
   from semi-supervised learning.
  %  TODO: Change this wording to emphasize novelty more novel ^^ 
   Intuitively, our work is based on the insight that in order to perform well on the target domain, a model’s output should be consistent with respect to small perturbations of inputs in the target domain. Specifically, we introduce a new loss term to enforce pixelwise consistency between the model's predictions on a target image and a heavily augmented version of the same image. In comparison to popular adversarial adaptation methods, our approach is both simpler and more stable during training. Experiments demonstrate that our approach achieves state-of-the-art performance on two challenging synthetic-to-real benchmarks, GTA5-to-Cityscapes and SYNTHIA-to-Cityscapes.
  \end{abstract}
  
  \section{Introduction}
  
  Deep neural network approaches for semantic image segmentation have shown widespread success in the past decade years, but they remain reliant on large datasets with pixel-level annotations. Data labeling for semantic segmentation is notoriously laborious and expensive, especially in domains where experts are required (e.g. medical image segmentation). Even for annotations that can be performed by non-experts like parsing an urban scene into familiar objects, as in the Cityscapes dataset \cite{cityscapes}, it takes an estimated 90 minutes to annotate a single image \cite{statistic}. 
  
  The need to build generalizable models with limited data has motivated work on unsupervised domain adaptation (UDA) approaches for semantic segmentation \cite{cbst,adaptsegnet,advent,maxsquare,cycada,chen2018road}, where annotated images from a simulated (source) domain, which are plentiful, are used in conjunction with unlabeled images from a real (target) domain. The simulated source domain in this ``synthetic to real'' translation task can be creative, such the video game Grand Theft Auto V in the GTA5-to-Cityscapes benchmark \cite{gta} and the simulation platform SYNTHIA as in the SYNTHIA-to-Cityscapes benchmark \cite{synthia}. 
  
  The literature on UDA for semantic segmentation is dominated by adversarial methods, which aim to learn domain-invariant representations across multiple domains by introducing adversarial losses \cite{cycada}. These methods have shown strong performance, but due to the instability of their adversarial losses, they are well-known to be highly sensitive to hyperparameters and difficult to train \cite{gans_hard_one,gans_hard_two,wgan}. 
  
  Recently, a new line of work on UDA for semantic segmentation has emerged around self-training \cite{cbst,advent,maxsquare}. These methods add loss terms to the training objective that encourage the segmentation model to make more confident predictions on the target domain (for example, by encouraging low-entropy predictions) \cite{advent,maxsquare,cbst}. 
  
  This paper begins with the observation that we do not simply desire a model that makes confident predictions in target domain, rather we desire a model that makes \textit{consistent} predictions in the target domain. That is, we desire a model for which small perturbations of inputs in the target domain lead to small, consistent changes in the output segmentation. If a model's predictions are always confident, but they are not stable with respect to small perturbations of target images, the model is likely to be poorly-adapted to the target domain. Conversely, if a model behaves smoothly with respect to perturbations of data in the target domain, it is intuitive that the model should be well-adapted to that domain. 
  
  In this paper, we propose a consistency training-based framework to directly enforce this notion of smoothness in the target domain. Our method, denoted PixMatch, adds a loss term that encourages the segmentation model's predictions on a target domain image and a perturbed version of the same image to be pixelwise consistent. 
  
  We experiment with four different perturbation functions, two of which are inspired by work in semi/self-supervised learning (Data Augmentations; CutMix) and two of which are inspired by work in domain adaptation (Style Transfer; Fourier Transfer). 
  
  Surprisingly, we find that our baseline model, which uses heavy data augmentation as its perturbation function, performs best. This simple baseline delivers extremely strong results on GTA5-to-Cityscapes \cite{cityscapes} and SYNTHIA-to-Cityscapes \cite{synthia}. 
  Using only a source (supervised) loss and a target consistency loss, it outperforms complex prior methods using combinations of source, adversarial, and self-training losses. 
  Compared to existing adversarial approaches, it is easier to implement, more stable during training, and less memory-intensive to train. It introduces only one hyperparameter, which controls the relative weighting of the source (supervised) loss and the target consistency loss. Moreover, the simplicity of PixMatch means that it it may be easily integrated into existing UDA methods and pipelines; combining PixMatch with self-training yields the state-of-the-art results. 
  
  
  
  
  % PixMatch achieves state of the art performance on two challenging synthetic-to-real benchmarks, GTA5-to-Cityscapes \cite{cityscapes} and SYNTHIA-to-Cityscapes \cite{synthia}. Using only a source (supervised) loss and a target consistency loss, PixMatch outperforms complex prior methods using combinations of source, adversarial, and self-training losses. Moreover, the simplicity of PixMatch means that it it may be easily integrated into existing UDA methods and pipelines; combining PixMatch with self-training yields further improvements over the state-of-the-art. 
  
  % (Data Augmentation; CutMix) 
  
  % We start by making the observation that these self-training approaches are rooted in classical semi-supervised learning methods \cite{selftrainingone,selftrainingtwo}. This 
  
  % This observation leads us to another classical 
  
  % , which has roots in the semi-supervised learning commmunity \cite{cotraining}
  
  % co-training, also called 
  
  
  % pseudolabeling and entropy minimization are two forms of \textit{self-training}, a classical method in the field of \emph{semi-supervised learning} (SSL). This observation leads to the question: can other ideas from SSL be employed for UDA?
  
  
  
  
  % In the past year, variants of these methods including have set state-of-the-art results, often by combining pseudolabeling and/or entropy minimization with adversarial approaches \cite{advent}. 
  
  % We start by making the observation that pseudolabeling and entropy minimization are two forms of \textit{self-training}, a classical method in the field of \emph{semi-supervised learning} (SSL). This observation leads to the question: can other ideas from SSL be employed for UDA?
  
  % We start by making the observation that self-training is a classical method in the field of semi/self-supervised learning, having been used as early as 
  
  % . This observation leads to the question: can other ideas from SSL be employed for UDA?
  
  
  % In the recent literature in SSL, methods based on \textit{consistency training} (also called \textit{consistency regularization}) have gained widespread adoption and shown remarkably strong performance using only a small number of labeled inputs \cite{xie2019unsupervised,berthelot2019mixmatch,berthelot2019mixmatch,fixmatch}. These methods encourage models to be consistent (i.e. produce the same output) on multiple views of the same input. In computer vision, this translates to adding a loss term that encourages a model's predictions on an image and a heavily-augmented version of the same image to be similar.
  
  
  
  %Using these methods, [cite UDA, MixMatch, ReMixMatch, FixMatch] show remarkably strong classification performance on image classification datasets (CIFAR-10, CIFAR-100, and ImageNet) using only a small number of labeled images.  
  
  % TODO: Add the references from the ssl section of the MSL paper (page 2, top, intro)
  
  % The nature and placement of the injected noise has proven crucial with the results striking, with approaches like Unsupervised Data Augmentation [cite] achieving an error rate of 2.7\% on the CIFAR-10 benchmark with only 4,000 examples. FixMatch [cite] combines the idea of consistency regularization with pseudo-labeling [cite] (self-training), achieving state of the art on a number of semi-supervised learning benchmarks.
  
  % A distinct line of work from the semi-supervised and self-supervised learning [cite] communities has shown the value of \emph{consistency training}, where model predictions for unlabeled data are regularized to be invariant to noise that is injected either in inputs [cite] or hidden states [cite]. The nature and placement of the injected noise has proven crucial with the results striking, with approaches like Unsupervised Data Augmentation [cite] achieving an error rate of 2.7\% on the CIFAR-10 benchmark with only 4,000 examples. FixMatch [cite] combines the idea of consistency regularization with pseudo-labeling [cite] (self-training), achieving state of the art on a number of semi-supervised learning benchmarks.
  
  % In this paper, we propose a consistency training-based method for unsupervised domain adaptation: PixMatch: Unsupervised Domain Adaptation via Pixelwise Consistency Training. Intuitively, our method reflects the idea that in order for a model to be well-adapted to a certain domain, it should make consistent predictions on multiple views of an input from that domain. Specifically, we add a loss term that encourages a semantic segmentation model's predictions on a target domain image and a heavily-augmented version of the same image to be pixelwise consistent. 
  
  % Our method is simple and non-adversarial. Compared to existing adversarial approaches, PixMatch is easier to implement, more stable during training, and less memory-intensive to train. It introduces only one hyperparameter, which controls the relative weighting of the source (supervised) loss and the target consistency loss. 
  
  % PixMatch achieves state of the art performance on two challenging synthetic-to-real benchmarks, GTA5-to-Cityscapes \cite{cityscapes} and SYNTHIA-to-Cityscapes \cite{synthia}. Using only a source (supervised) loss and a target consistency loss, PixMatch outperforms complex prior methods using combinations of source, adversarial, and self-training losses. Moreover, the simplicity of PixMatch means that it it may be easily integrated into existing UDA methods and pipelines; combining PixMatch with self-training yields further improvements over the state-of-the-art. 
  
  The main contributions of this paper are:
  
  \begin{itemize}
  \item We introduce a consistency-based method for unsupervised domain adaptation that encourages pixelwise consistency between a model's predictions on a target image and a heavily augmented version of the same image.
  \item We achieve a new state-of-the-art in unsupervised domain adaptation for semantic segmentation for both the GTA5-to-Cityscapes and SYNTHIA-to-Cityscapes benchmarks with a simpler training approach than comparable adversarial approaches.
  \item We perform extensive ablation studies on our method, examining its sensitivity to different types of data augmentations and across various parameter settings. We find that out model may be easily combined with self-labeling for further performance improvements.
  % \item We show how semi-supervised learning methods can be applied more broadly to improve semantic segmentation.
  \end{itemize}
  
  
